Enhancing Code Translation in Language Models with Few-Shot Learning via Retrieval-Augmented Generation

The advent of large language models (LLMs) has significantly advanced the field of code translation, enabling automated translation between programming languages. However, these models often struggle with complex translation tasks due to inadequate contextual understanding. This paper introduces a novel approach that enhances code translation through Few-Shot Learning, augmented with retrieval-based techniques. By leveraging a repository of existing code translations, we dynamically retrieve the most relevant examples to guide the model in translating new code segments. Our method, based on Retrieval-Augmented Generation (RAG), substantially improves translation quality by providing contextual examples from which the model can learn in real-time. We selected RAG over traditional fine-tuning methods due to its ability to utilize existing codebases or a locally stored corpus of code, which allows for dynamic adaptation to diverse translation tasks without extensive retraining. Extensive experiments on diverse datasets with open LLM models such as Starcoder, Llama3-70B Instruct, CodeLlama-34B Instruct, Granite-34B Code Instruct, and Mixtral-8x22B, as well as commercial LLM models like GPT-3.5 Turbo and GPT-4o, demonstrate our approach's superiority over traditional zero-shot methods, especially in translating between Fortran and CPP. We also explored varying numbers of shots i.e. examples provided during inference, specifically 1, 2, and 3 shots and different embedding models for RAG, including Nomic-Embed, Starencoder, and CodeBERT, to assess the robustness and effectiveness of our approach.

==> table <==
\begin{tabular}{llllllllrlllll}
\toprule
          Dataset &              Model & Embedding Model & Zero-shot CodeBLEU & Zero-shot Ngram Match & Zero-shot Weighted Ngram & Zero-shot Syntax Match & Zero-shot Dataflow Match &  Shots & One-shot CodeBLEU & One-shot Ngram Match & One-shot Weighted Ngram & One-shot Syntax Match & One-shot Dataflow Match \\
\midrule
             llnl &       codellama34b &        codebert &        0.24 ± 0.09 &           0.09 ± 0.09 &              0.16 ± 0.13 &            0.17 ± 0.14 &              0.49 ± 0.27 &      1 &       0.33 ± 0.16 &          0.17 ± 0.17 &             0.24 ± 0.20 &           0.33 ± 0.25 &             0.52 ± 0.28 \\
             llnl &       codellama34b &        codebert &        0.24 ± 0.09 &           0.09 ± 0.09 &              0.16 ± 0.13 &            0.17 ± 0.14 &              0.49 ± 0.27 &      2 &       0.32 ± 0.16 &          0.16 ± 0.17 &             0.23 ± 0.20 &           0.32 ± 0.24 &             0.53 ± 0.28 \\
             llnl &       codellama34b &        codebert &        0.24 ± 0.09 &           0.09 ± 0.09 &              0.16 ± 0.13 &            0.17 ± 0.14 &              0.49 ± 0.27 &      3 &       0.31 ± 0.14 &          0.16 ± 0.15 &             0.23 ± 0.19 &           0.31 ± 0.23 &             0.51 ± 0.27 \\
             llnl &       codellama34b &     nomic_embed &        0.24 ± 0.09 &           0.09 ± 0.09 &              0.17 ± 0.14 &            0.17 ± 0.14 &              0.49 ± 0.28 &      1 &       0.32 ± 0.15 &          0.16 ± 0.16 &             0.24 ± 0.19 &           0.32 ± 0.24 &             0.51 ± 0.29 \\
             llnl &       codellama34b &     nomic_embed &        0.24 ± 0.09 &           0.09 ± 0.09 &              0.17 ± 0.14 &            0.17 ± 0.14 &              0.49 ± 0.28 &      2 &       0.33 ± 0.16 &          0.16 ± 0.17 &             0.24 ± 0.20 &           0.33 ± 0.25 &             0.52 ± 0.29 \\
             llnl &       codellama34b &     nomic_embed &        0.24 ± 0.09 &           0.09 ± 0.09 &              0.17 ± 0.14 &            0.17 ± 0.14 &              0.49 ± 0.28 &      3 &       0.31 ± 0.14 &          0.15 ± 0.15 &             0.23 ± 0.18 &           0.32 ± 0.23 &             0.51 ± 0.28 \\
             llnl &       codellama34b &     starencoder &        0.24 ± 0.09 &           0.09 ± 0.09 &              0.16 ± 0.14 &            0.16 ± 0.14 &              0.49 ± 0.28 &      1 &       0.32 ± 0.15 &          0.16 ± 0.16 &             0.23 ± 0.19 &           0.33 ± 0.25 &             0.52 ± 0.28 \\
             llnl &       codellama34b &     starencoder &        0.24 ± 0.09 &           0.09 ± 0.09 &              0.16 ± 0.14 &            0.16 ± 0.14 &              0.49 ± 0.28 &      2 &       0.33 ± 0.15 &          0.16 ± 0.16 &             0.23 ± 0.19 &           0.33 ± 0.25 &             0.54 ± 0.28 \\
             llnl &       codellama34b &     starencoder &        0.24 ± 0.09 &           0.09 ± 0.09 &              0.16 ± 0.14 &            0.16 ± 0.14 &              0.49 ± 0.28 &      3 &       0.32 ± 0.14 &          0.16 ± 0.15 &             0.23 ± 0.19 &           0.32 ± 0.24 &             0.54 ± 0.28 \\
             llnl &        granite-34b &        codebert &        0.24 ± 0.09 &           0.09 ± 0.09 &              0.14 ± 0.13 &            0.17 ± 0.13 &              0.51 ± 0.26 &      1 &       0.58 ± 0.27 &          0.45 ± 0.31 &             0.49 ± 0.31 &           0.61 ± 0.35 &             0.70 ± 0.33 \\
             llnl &        granite-34b &        codebert &        0.24 ± 0.09 &           0.09 ± 0.09 &              0.14 ± 0.13 &            0.17 ± 0.13 &              0.51 ± 0.26 &      2 &       0.52 ± 0.27 &          0.41 ± 0.31 &             0.44 ± 0.30 &           0.55 ± 0.35 &             0.62 ± 0.34 \\
             llnl &        granite-34b &        codebert &        0.24 ± 0.09 &           0.09 ± 0.09 &              0.14 ± 0.13 &            0.17 ± 0.13 &              0.51 ± 0.26 &      3 &       0.54 ± 0.27 &          0.43 ± 0.30 &             0.47 ± 0.30 &           0.56 ± 0.35 &             0.64 ± 0.33 \\
             llnl &        granite-34b &     nomic_embed &        0.24 ± 0.09 &           0.08 ± 0.08 &              0.15 ± 0.13 &            0.17 ± 0.14 &              0.50 ± 0.27 &      1 &       0.60 ± 0.27 &          0.47 ± 0.32 &             0.51 ± 0.31 &           0.63 ± 0.34 &             0.72 ± 0.33 \\
             llnl &        granite-34b &     nomic_embed &        0.24 ± 0.09 &           0.08 ± 0.08 &              0.15 ± 0.13 &            0.17 ± 0.14 &              0.50 ± 0.27 &      2 &       0.51 ± 0.28 &          0.40 ± 0.31 &             0.44 ± 0.31 &           0.52 ± 0.37 &             0.64 ± 0.34 \\
             llnl &        granite-34b &     nomic_embed &        0.24 ± 0.09 &           0.08 ± 0.08 &              0.15 ± 0.13 &            0.17 ± 0.14 &              0.50 ± 0.27 &      3 &       0.54 ± 0.27 &          0.43 ± 0.31 &             0.47 ± 0.31 &           0.54 ± 0.36 &             0.64 ± 0.35 \\
             llnl &        granite-34b &     starencoder &        0.24 ± 0.09 &           0.08 ± 0.08 &              0.14 ± 0.13 &            0.17 ± 0.14 &              0.51 ± 0.26 &      1 &       0.60 ± 0.27 &          0.47 ± 0.31 &             0.50 ± 0.31 &           0.63 ± 0.34 &             0.73 ± 0.32 \\
             llnl &        granite-34b &     starencoder &        0.24 ± 0.09 &           0.08 ± 0.08 &              0.14 ± 0.13 &            0.17 ± 0.14 &              0.51 ± 0.26 &      2 &       0.54 ± 0.28 &          0.42 ± 0.32 &             0.45 ± 0.32 &           0.55 ± 0.36 &             0.66 ± 0.33 \\
             llnl &        granite-34b &     starencoder &        0.24 ± 0.09 &           0.08 ± 0.08 &              0.14 ± 0.13 &            0.17 ± 0.14 &              0.51 ± 0.26 &      3 &       0.52 ± 0.27 &          0.42 ± 0.31 &             0.45 ± 0.30 &           0.53 ± 0.35 &             0.64 ± 0.33 \\
             llnl & llama3b70-instruct &        codebert &        0.24 ± 0.08 &           0.07 ± 0.07 &              0.14 ± 0.12 &            0.16 ± 0.14 &              0.53 ± 0.28 &      1 &       0.28 ± 0.11 &          0.12 ± 0.12 &             0.18 ± 0.16 &           0.25 ± 0.21 &             0.49 ± 0.28 \\
             llnl & llama3b70-instruct &        codebert &        0.24 ± 0.08 &           0.07 ± 0.07 &              0.14 ± 0.12 &            0.16 ± 0.14 &              0.53 ± 0.28 &      2 &       0.31 ± 0.13 &          0.16 ± 0.14 &             0.22 ± 0.17 &           0.30 ± 0.22 &             0.50 ± 0.27 \\
             llnl & llama3b70-instruct &        codebert &        0.24 ± 0.08 &           0.07 ± 0.07 &              0.14 ± 0.12 &            0.16 ± 0.14 &              0.53 ± 0.28 &      3 &       0.29 ± 0.12 &          0.15 ± 0.13 &             0.20 ± 0.17 &           0.27 ± 0.21 &             0.50 ± 0.28 \\
             llnl & llama3b70-instruct &     nomic_embed &        0.24 ± 0.08 &           0.07 ± 0.07 &              0.13 ± 0.13 &            0.16 ± 0.14 &              0.52 ± 0.28 &      1 &       0.27 ± 0.11 &          0.12 ± 0.12 &             0.18 ± 0.15 &           0.25 ± 0.20 &             0.49 ± 0.29 \\
             llnl & llama3b70-instruct &     nomic_embed &        0.24 ± 0.08 &           0.07 ± 0.07 &              0.13 ± 0.13 &            0.16 ± 0.14 &              0.52 ± 0.28 &      2 &       0.29 ± 0.11 &          0.13 ± 0.13 &             0.19 ± 0.16 &           0.26 ± 0.20 &             0.49 ± 0.29 \\
             llnl & llama3b70-instruct &     nomic_embed &        0.24 ± 0.08 &           0.07 ± 0.07 &              0.13 ± 0.13 &            0.16 ± 0.14 &              0.52 ± 0.28 &      3 &       0.29 ± 0.12 &          0.14 ± 0.13 &             0.20 ± 0.17 &           0.28 ± 0.21 &             0.49 ± 0.28 \\
             llnl & llama3b70-instruct &     starencoder &        0.24 ± 0.08 &           0.07 ± 0.07 &              0.13 ± 0.12 &            0.16 ± 0.14 &              0.53 ± 0.29 &      1 &       0.27 ± 0.10 &          0.10 ± 0.11 &             0.16 ± 0.15 &           0.23 ± 0.19 &             0.49 ± 0.30 \\
             llnl & llama3b70-instruct &     starencoder &        0.24 ± 0.08 &           0.07 ± 0.07 &              0.13 ± 0.12 &            0.16 ± 0.14 &              0.53 ± 0.29 &      2 &       0.30 ± 0.12 &          0.15 ± 0.13 &             0.21 ± 0.17 &           0.29 ± 0.21 &             0.51 ± 0.28 \\
             llnl & llama3b70-instruct &     starencoder &        0.24 ± 0.08 &           0.07 ± 0.07 &              0.13 ± 0.12 &            0.16 ± 0.14 &              0.53 ± 0.29 &      3 &       0.28 ± 0.11 &          0.13 ± 0.12 &             0.18 ± 0.16 &           0.24 ± 0.20 &             0.50 ± 0.28 \\
             llnl &      mixtral-8x22b &        codebert &        0.24 ± 0.10 &           0.06 ± 0.06 &              0.10 ± 0.11 &            0.14 ± 0.13 &              0.33 ± 0.33 &      1 &       0.51 ± 0.29 &          0.39 ± 0.35 &             0.42 ± 0.35 &           0.48 ± 0.36 &             0.60 ± 0.39 \\
             llnl &      mixtral-8x22b &        codebert &        0.24 ± 0.10 &           0.06 ± 0.06 &              0.10 ± 0.11 &            0.14 ± 0.13 &              0.33 ± 0.33 &      2 &       0.53 ± 0.27 &          0.40 ± 0.34 &             0.43 ± 0.34 &           0.51 ± 0.36 &             0.66 ± 0.37 \\
             llnl &      mixtral-8x22b &        codebert &        0.24 ± 0.10 &           0.06 ± 0.06 &              0.10 ± 0.11 &            0.14 ± 0.13 &              0.33 ± 0.33 &      3 &       0.55 ± 0.28 &          0.42 ± 0.36 &             0.44 ± 0.35 &           0.52 ± 0.38 &             0.65 ± 0.38 \\
             llnl &      mixtral-8x22b &     nomic_embed &        0.24 ± 0.10 &           0.06 ± 0.06 &              0.11 ± 0.12 &            0.14 ± 0.14 &              0.33 ± 0.33 &      1 &       0.51 ± 0.29 &          0.39 ± 0.34 &             0.42 ± 0.35 &           0.49 ± 0.38 &             0.60 ± 0.39 \\
             llnl &      mixtral-8x22b &     nomic_embed &        0.24 ± 0.10 &           0.06 ± 0.06 &              0.11 ± 0.12 &            0.14 ± 0.14 &              0.33 ± 0.33 &      2 &       0.59 ± 0.26 &          0.45 ± 0.33 &             0.48 ± 0.32 &           0.58 ± 0.36 &             0.71 ± 0.36 \\
             llnl &      mixtral-8x22b &     nomic_embed &        0.24 ± 0.10 &           0.06 ± 0.06 &              0.11 ± 0.12 &            0.14 ± 0.14 &              0.33 ± 0.33 &      3 &       0.60 ± 0.26 &          0.47 ± 0.33 &             0.50 ± 0.33 &           0.60 ± 0.34 &             0.70 ± 0.35 \\
             llnl &      mixtral-8x22b &     starencoder &        0.24 ± 0.10 &           0.06 ± 0.06 &              0.10 ± 0.11 &            0.14 ± 0.13 &              0.33 ± 0.33 &      1 &       0.52 ± 0.28 &          0.38 ± 0.34 &             0.41 ± 0.35 &           0.49 ± 0.37 &             0.63 ± 0.39 \\
             llnl &      mixtral-8x22b &     starencoder &        0.24 ± 0.10 &           0.06 ± 0.06 &              0.10 ± 0.11 &            0.14 ± 0.13 &              0.33 ± 0.33 &      2 &       0.55 ± 0.29 &          0.42 ± 0.35 &             0.45 ± 0.34 &           0.54 ± 0.36 &             0.68 ± 0.37 \\
             llnl &      mixtral-8x22b &     starencoder &        0.24 ± 0.10 &           0.06 ± 0.06 &              0.10 ± 0.11 &            0.14 ± 0.13 &              0.33 ± 0.33 &      3 &       0.57 ± 0.27 &          0.44 ± 0.34 &             0.47 ± 0.34 &           0.54 ± 0.37 &             0.65 ± 0.38 \\
             llnl &               phi3 &        codebert &        0.23 ± 0.08 &           0.08 ± 0.07 &              0.14 ± 0.12 &            0.16 ± 0.14 &              0.51 ± 0.27 &      1 &       0.29 ± 0.12 &          0.11 ± 0.10 &             0.20 ± 0.15 &           0.25 ± 0.21 &             0.55 ± 0.30 \\
             llnl &               phi3 &        codebert &        0.23 ± 0.08 &           0.08 ± 0.07 &              0.14 ± 0.12 &            0.16 ± 0.14 &              0.51 ± 0.27 &      2 &       0.31 ± 0.13 &          0.13 ± 0.13 &             0.21 ± 0.17 &           0.28 ± 0.21 &             0.55 ± 0.29 \\
             llnl &               phi3 &     nomic_embed &        0.23 ± 0.08 &           0.08 ± 0.07 &              0.14 ± 0.12 &            0.16 ± 0.14 &              0.50 ± 0.27 &      1 &       0.29 ± 0.11 &          0.11 ± 0.10 &             0.20 ± 0.15 &           0.24 ± 0.19 &             0.55 ± 0.30 \\
             llnl &               phi3 &     nomic_embed &        0.23 ± 0.08 &           0.08 ± 0.07 &              0.14 ± 0.12 &            0.16 ± 0.14 &              0.50 ± 0.27 &      2 &       0.31 ± 0.13 &          0.13 ± 0.13 &             0.21 ± 0.17 &           0.29 ± 0.21 &             0.55 ± 0.29 \\
             llnl &               phi3 &     starencoder &        0.23 ± 0.08 &           0.08 ± 0.07 &              0.14 ± 0.12 &            0.16 ± 0.14 &              0.51 ± 0.27 &      1 &       0.29 ± 0.11 &          0.11 ± 0.10 &             0.19 ± 0.15 &           0.25 ± 0.21 &             0.54 ± 0.30 \\
             llnl &               phi3 &     starencoder &        0.23 ± 0.08 &           0.08 ± 0.07 &              0.14 ± 0.12 &            0.16 ± 0.14 &              0.51 ± 0.27 &      2 &       0.32 ± 0.14 &          0.14 ± 0.14 &             0.22 ± 0.18 &           0.31 ± 0.23 &             0.55 ± 0.29 \\
             llnl &               phi3 &     starencoder &        0.23 ± 0.08 &           0.08 ± 0.07 &              0.14 ± 0.12 &            0.16 ± 0.14 &              0.51 ± 0.27 &      3 &       0.31 ± 0.15 &          0.14 ± 0.16 &             0.21 ± 0.19 &           0.29 ± 0.22 &             0.57 ± 0.28 \\
             llnl &          starcoder &        codebert &        0.21 ± 0.07 &           0.01 ± 0.01 &              0.01 ± 0.01 &            0.12 ± 0.11 &              0.65 ± 0.30 &      1 &       0.21 ± 0.07 &          0.01 ± 0.01 &             0.01 ± 0.01 &           0.12 ± 0.11 &             0.64 ± 0.30 \\
             llnl &          starcoder &        codebert &        0.21 ± 0.07 &           0.01 ± 0.01 &              0.01 ± 0.01 &            0.12 ± 0.11 &              0.65 ± 0.30 &      2 &       0.21 ± 0.06 &          0.01 ± 0.01 &             0.01 ± 0.01 &           0.12 ± 0.10 &             0.65 ± 0.29 \\
             llnl &          starcoder &        codebert &        0.21 ± 0.07 &           0.01 ± 0.01 &              0.01 ± 0.01 &            0.12 ± 0.11 &              0.65 ± 0.30 &      3 &       0.21 ± 0.06 &          0.01 ± 0.01 &             0.01 ± 0.01 &           0.12 ± 0.10 &             0.65 ± 0.29 \\
             llnl &          starcoder &     nomic_embed &        0.21 ± 0.07 &           0.01 ± 0.01 &              0.01 ± 0.01 &            0.13 ± 0.11 &              0.63 ± 0.31 &      1 &       0.21 ± 0.07 &          0.01 ± 0.01 &             0.01 ± 0.01 &           0.13 ± 0.11 &             0.63 ± 0.31 \\
             llnl &          starcoder &     nomic_embed &        0.21 ± 0.07 &           0.01 ± 0.01 &              0.01 ± 0.01 &            0.13 ± 0.11 &              0.63 ± 0.31 &      2 &       0.21 ± 0.07 &          0.01 ± 0.01 &             0.01 ± 0.01 &           0.12 ± 0.11 &             0.63 ± 0.31 \\
             llnl &          starcoder &     nomic_embed &        0.21 ± 0.07 &           0.01 ± 0.01 &              0.01 ± 0.01 &            0.13 ± 0.11 &              0.63 ± 0.31 &      3 &       0.21 ± 0.07 &          0.01 ± 0.01 &             0.01 ± 0.01 &           0.13 ± 0.11 &             0.63 ± 0.30 \\
             llnl &          starcoder &     starencoder &        0.21 ± 0.07 &           0.01 ± 0.01 &              0.01 ± 0.01 &            0.12 ± 0.11 &              0.65 ± 0.30 &      1 &       0.21 ± 0.07 &          0.01 ± 0.01 &             0.01 ± 0.01 &           0.12 ± 0.11 &             0.63 ± 0.31 \\
             llnl &          starcoder &     starencoder &        0.21 ± 0.07 &           0.01 ± 0.01 &              0.01 ± 0.01 &            0.12 ± 0.11 &              0.65 ± 0.30 &      2 &       0.21 ± 0.06 &          0.01 ± 0.01 &             0.01 ± 0.01 &           0.12 ± 0.11 &             0.65 ± 0.30 \\
             llnl &          starcoder &     starencoder &        0.21 ± 0.07 &           0.01 ± 0.01 &              0.01 ± 0.01 &            0.12 ± 0.11 &              0.65 ± 0.30 &      3 &       0.21 ± 0.06 &          0.01 ± 0.01 &             0.01 ± 0.01 &           0.12 ± 0.11 &             0.65 ± 0.29 \\
numerical_receipe &       codellama34b &        codebert &        0.28 ± 0.07 &           0.03 ± 0.04 &              0.11 ± 0.09 &            0.48 ± 0.17 &              0.48 ± 0.16 &      1 &       0.41 ± 0.19 &          0.23 ± 0.22 &             0.34 ± 0.22 &           0.59 ± 0.22 &             0.50 ± 0.23 \\
numerical_receipe &       codellama34b &        codebert &        0.28 ± 0.07 &           0.03 ± 0.04 &              0.11 ± 0.09 &            0.48 ± 0.17 &              0.48 ± 0.16 &      2 &       0.44 ± 0.20 &          0.28 ± 0.24 &             0.37 ± 0.24 &           0.60 ± 0.22 &             0.52 ± 0.23 \\
numerical_receipe &       codellama34b &        codebert &        0.28 ± 0.07 &           0.03 ± 0.04 &              0.11 ± 0.09 &            0.48 ± 0.17 &              0.48 ± 0.16 &      3 &       0.42 ± 0.19 &          0.26 ± 0.23 &             0.34 ± 0.23 &           0.60 ± 0.22 &             0.49 ± 0.21 \\
numerical_receipe &       codellama34b &     nomic_embed &        0.28 ± 0.07 &           0.03 ± 0.04 &              0.11 ± 0.09 &            0.48 ± 0.17 &              0.49 ± 0.17 &      1 &       0.42 ± 0.19 &          0.24 ± 0.22 &             0.35 ± 0.23 &           0.60 ± 0.22 &             0.51 ± 0.22 \\
numerical_receipe &       codellama34b &     nomic_embed &        0.28 ± 0.07 &           0.03 ± 0.04 &              0.11 ± 0.09 &            0.48 ± 0.17 &              0.49 ± 0.17 &      2 &       0.44 ± 0.18 &          0.26 ± 0.23 &             0.37 ± 0.22 &           0.61 ± 0.21 &             0.51 ± 0.22 \\
numerical_receipe &       codellama34b &     nomic_embed &        0.28 ± 0.07 &           0.03 ± 0.04 &              0.11 ± 0.09 &            0.48 ± 0.17 &              0.49 ± 0.17 &      3 &       0.42 ± 0.20 &          0.27 ± 0.25 &             0.36 ± 0.24 &           0.58 ± 0.23 &             0.48 ± 0.23 \\
numerical_receipe &       codellama34b &     starencoder &        0.28 ± 0.07 &           0.03 ± 0.04 &              0.11 ± 0.08 &            0.47 ± 0.17 &              0.49 ± 0.17 &      1 &       0.46 ± 0.19 &          0.28 ± 0.24 &             0.39 ± 0.24 &           0.63 ± 0.22 &             0.53 ± 0.23 \\
numerical_receipe &       codellama34b &     starencoder &        0.28 ± 0.07 &           0.03 ± 0.04 &              0.11 ± 0.08 &            0.47 ± 0.17 &              0.49 ± 0.17 &      2 &       0.45 ± 0.20 &          0.30 ± 0.24 &             0.40 ± 0.24 &           0.61 ± 0.22 &             0.51 ± 0.23 \\
numerical_receipe &       codellama34b &     starencoder &        0.28 ± 0.07 &           0.03 ± 0.04 &              0.11 ± 0.08 &            0.47 ± 0.17 &              0.49 ± 0.17 &      3 &       0.44 ± 0.19 &          0.26 ± 0.22 &             0.37 ± 0.23 &           0.59 ± 0.22 &             0.52 ± 0.22 \\
numerical_receipe &        granite-34b &        codebert &        0.27 ± 0.11 &           0.06 ± 0.09 &              0.11 ± 0.11 &            0.45 ± 0.20 &              0.44 ± 0.19 &      1 &       0.49 ± 0.20 &          0.36 ± 0.25 &             0.40 ± 0.25 &           0.67 ± 0.18 &             0.52 ± 0.23 \\
numerical_receipe &        granite-34b &        codebert &        0.27 ± 0.11 &           0.06 ± 0.09 &              0.11 ± 0.11 &            0.45 ± 0.20 &              0.44 ± 0.19 &      2 &       0.51 ± 0.21 &          0.39 ± 0.25 &             0.43 ± 0.25 &           0.69 ± 0.19 &             0.54 ± 0.23 \\
numerical_receipe &        granite-34b &        codebert &        0.27 ± 0.11 &           0.06 ± 0.09 &              0.11 ± 0.11 &            0.45 ± 0.20 &              0.44 ± 0.19 &      3 &       0.52 ± 0.22 &          0.40 ± 0.27 &             0.44 ± 0.26 &           0.69 ± 0.19 &             0.55 ± 0.24 \\
numerical_receipe &        granite-34b &     nomic_embed &        0.27 ± 0.11 &           0.06 ± 0.09 &              0.11 ± 0.11 &            0.46 ± 0.19 &              0.44 ± 0.19 &      1 &       0.50 ± 0.19 &          0.37 ± 0.24 &             0.41 ± 0.24 &           0.68 ± 0.18 &             0.53 ± 0.23 \\
numerical_receipe &        granite-34b &     nomic_embed &        0.27 ± 0.11 &           0.06 ± 0.09 &              0.11 ± 0.11 &            0.46 ± 0.19 &              0.44 ± 0.19 &      2 &       0.51 ± 0.21 &          0.39 ± 0.25 &             0.43 ± 0.25 &           0.69 ± 0.19 &             0.54 ± 0.24 \\
numerical_receipe &        granite-34b &     nomic_embed &        0.27 ± 0.11 &           0.06 ± 0.09 &              0.11 ± 0.11 &            0.46 ± 0.19 &              0.44 ± 0.19 &      3 &       0.53 ± 0.21 &          0.41 ± 0.26 &             0.44 ± 0.25 &           0.70 ± 0.18 &             0.55 ± 0.24 \\
numerical_receipe &        granite-34b &     starencoder &        0.27 ± 0.11 &           0.06 ± 0.10 &              0.11 ± 0.11 &            0.45 ± 0.20 &              0.44 ± 0.19 &      1 &       0.52 ± 0.20 &          0.40 ± 0.25 &             0.44 ± 0.24 &           0.69 ± 0.18 &             0.53 ± 0.23 \\
numerical_receipe &        granite-34b &     starencoder &        0.27 ± 0.11 &           0.06 ± 0.10 &              0.11 ± 0.11 &            0.45 ± 0.20 &              0.44 ± 0.19 &      2 &       0.53 ± 0.21 &          0.42 ± 0.26 &             0.45 ± 0.25 &           0.70 ± 0.18 &             0.56 ± 0.24 \\
numerical_receipe &        granite-34b &     starencoder &        0.27 ± 0.11 &           0.06 ± 0.10 &              0.11 ± 0.11 &            0.45 ± 0.20 &              0.44 ± 0.19 &      3 &       0.54 ± 0.21 &          0.43 ± 0.26 &             0.47 ± 0.25 &           0.71 ± 0.18 &             0.55 ± 0.24 \\
numerical_receipe & llama3b70-instruct &        codebert &        0.29 ± 0.07 &           0.04 ± 0.04 &              0.11 ± 0.09 &            0.52 ± 0.15 &              0.49 ± 0.15 &      1 &       0.44 ± 0.16 &          0.24 ± 0.20 &             0.36 ± 0.22 &           0.65 ± 0.19 &             0.50 ± 0.19 \\
numerical_receipe & llama3b70-instruct &        codebert &        0.29 ± 0.07 &           0.04 ± 0.04 &              0.11 ± 0.09 &            0.52 ± 0.15 &              0.49 ± 0.15 &      2 &       0.45 ± 0.18 &          0.27 ± 0.23 &             0.37 ± 0.23 &           0.65 ± 0.20 &             0.53 ± 0.21 \\
numerical_receipe & llama3b70-instruct &        codebert &        0.29 ± 0.07 &           0.04 ± 0.04 &              0.11 ± 0.09 &            0.52 ± 0.15 &              0.49 ± 0.15 &      3 &       0.45 ± 0.17 &          0.28 ± 0.21 &             0.37 ± 0.22 &           0.64 ± 0.19 &             0.52 ± 0.20 \\
numerical_receipe & llama3b70-instruct &     nomic_embed &        0.28 ± 0.06 &           0.04 ± 0.04 &              0.10 ± 0.09 &            0.51 ± 0.15 &              0.48 ± 0.15 &      1 &       0.43 ± 0.17 &          0.24 ± 0.20 &             0.35 ± 0.22 &           0.65 ± 0.20 &             0.49 ± 0.20 \\
numerical_receipe & llama3b70-instruct &     nomic_embed &        0.28 ± 0.06 &           0.04 ± 0.04 &              0.10 ± 0.09 &            0.51 ± 0.15 &              0.48 ± 0.15 &      2 &       0.45 ± 0.17 &          0.26 ± 0.22 &             0.36 ± 0.22 &           0.67 ± 0.19 &             0.51 ± 0.20 \\
numerical_receipe & llama3b70-instruct &     nomic_embed &        0.28 ± 0.06 &           0.04 ± 0.04 &              0.10 ± 0.09 &            0.51 ± 0.15 &              0.48 ± 0.15 &      3 &       0.45 ± 0.17 &          0.28 ± 0.22 &             0.37 ± 0.23 &           0.65 ± 0.20 &             0.50 ± 0.19 \\
numerical_receipe & llama3b70-instruct &     starencoder &        0.29 ± 0.07 &           0.04 ± 0.04 &              0.11 ± 0.09 &            0.51 ± 0.16 &              0.49 ± 0.15 &      1 &       0.47 ± 0.18 &          0.28 ± 0.23 &             0.40 ± 0.24 &           0.67 ± 0.19 &             0.52 ± 0.20 \\
numerical_receipe & llama3b70-instruct &     starencoder &        0.29 ± 0.07 &           0.04 ± 0.04 &              0.11 ± 0.09 &            0.51 ± 0.16 &              0.49 ± 0.15 &      2 &       0.46 ± 0.18 &          0.28 ± 0.23 &             0.39 ± 0.23 &           0.67 ± 0.19 &             0.51 ± 0.20 \\
numerical_receipe & llama3b70-instruct &     starencoder &        0.29 ± 0.07 &           0.04 ± 0.04 &              0.11 ± 0.09 &            0.51 ± 0.16 &              0.49 ± 0.15 &      3 &       0.47 ± 0.18 &          0.29 ± 0.23 &             0.39 ± 0.23 &           0.66 ± 0.20 &             0.52 ± 0.21 \\
numerical_receipe &      mixtral-8x22b &        codebert &        0.25 ± 0.01 &           0.00 ± 0.02 &              0.00 ± 0.03 &            0.01 ± 0.08 &              0.01 ± 0.08 &      1 &       0.38 ± 0.22 &          0.20 ± 0.28 &             0.23 ± 0.29 &           0.36 ± 0.37 &             0.30 ± 0.33 \\
numerical_receipe &      mixtral-8x22b &        codebert &        0.25 ± 0.01 &           0.00 ± 0.02 &              0.00 ± 0.03 &            0.01 ± 0.08 &              0.01 ± 0.08 &      2 &       0.50 ± 0.21 &          0.35 ± 0.27 &             0.39 ± 0.27 &           0.64 ± 0.26 &             0.53 ± 0.26 \\
numerical_receipe &      mixtral-8x22b &        codebert &        0.25 ± 0.01 &           0.00 ± 0.02 &              0.00 ± 0.03 &            0.01 ± 0.08 &              0.01 ± 0.08 &      3 &       0.41 ± 0.22 &          0.24 ± 0.27 &             0.30 ± 0.27 &           0.51 ± 0.31 &             0.45 ± 0.29 \\
numerical_receipe &      mixtral-8x22b &     nomic_embed &        0.25 ± 0.02 &           0.00 ± 0.02 &              0.00 ± 0.03 &            0.01 ± 0.05 &              0.01 ± 0.06 &      1 &       0.41 ± 0.21 &          0.25 ± 0.28 &             0.27 ± 0.29 &           0.39 ± 0.36 &             0.34 ± 0.35 \\
numerical_receipe &      mixtral-8x22b &     nomic_embed &        0.25 ± 0.02 &           0.00 ± 0.02 &              0.00 ± 0.03 &            0.01 ± 0.05 &              0.01 ± 0.06 &      2 &       0.50 ± 0.22 &          0.37 ± 0.28 &             0.40 ± 0.29 &           0.59 ± 0.30 &             0.47 ± 0.31 \\
numerical_receipe &      mixtral-8x22b &     nomic_embed &        0.25 ± 0.02 &           0.00 ± 0.02 &              0.00 ± 0.03 &            0.01 ± 0.05 &              0.01 ± 0.06 &      3 &       0.45 ± 0.21 &          0.31 ± 0.27 &             0.34 ± 0.27 &           0.59 ± 0.30 &             0.44 ± 0.28 \\
numerical_receipe &      mixtral-8x22b &     starencoder &        0.25 ± 0.02 &           0.00 ± 0.01 &              0.00 ± 0.02 &            0.02 ± 0.10 &              0.03 ± 0.10 &      1 &       0.42 ± 0.21 &          0.26 ± 0.28 &             0.28 ± 0.29 &           0.44 ± 0.38 &             0.32 ± 0.31 \\
numerical_receipe &      mixtral-8x22b &     starencoder &        0.25 ± 0.02 &           0.00 ± 0.01 &              0.00 ± 0.02 &            0.02 ± 0.10 &              0.03 ± 0.10 &      2 &       0.53 ± 0.23 &          0.41 ± 0.28 &             0.46 ± 0.29 &           0.66 ± 0.27 &             0.50 ± 0.29 \\
numerical_receipe &      mixtral-8x22b &     starencoder &        0.25 ± 0.02 &           0.00 ± 0.01 &              0.00 ± 0.02 &            0.02 ± 0.10 &              0.03 ± 0.10 &      3 &       0.51 ± 0.22 &          0.38 ± 0.29 &             0.42 ± 0.29 &           0.63 ± 0.28 &             0.52 ± 0.30 \\
numerical_receipe &               phi3 &        codebert &        0.25 ± 0.08 &           0.04 ± 0.04 &              0.09 ± 0.08 &            0.44 ± 0.16 &              0.44 ± 0.17 &      1 &       0.31 ± 0.12 &          0.09 ± 0.11 &             0.19 ± 0.15 &           0.50 ± 0.18 &             0.45 ± 0.20 \\
numerical_receipe &               phi3 &        codebert &        0.25 ± 0.08 &           0.04 ± 0.04 &              0.09 ± 0.08 &            0.44 ± 0.16 &              0.44 ± 0.17 &      2 &       0.29 ± 0.11 &          0.07 ± 0.07 &             0.18 ± 0.14 &           0.45 ± 0.19 &             0.46 ± 0.21 \\
numerical_receipe &               phi3 &     nomic_embed &        0.25 ± 0.08 &           0.04 ± 0.04 &              0.09 ± 0.08 &            0.44 ± 0.16 &              0.44 ± 0.17 &      1 &       0.32 ± 0.12 &          0.10 ± 0.12 &             0.21 ± 0.16 &           0.52 ± 0.17 &             0.46 ± 0.18 \\
numerical_receipe &               phi3 &     nomic_embed &        0.25 ± 0.08 &           0.04 ± 0.04 &              0.09 ± 0.08 &            0.44 ± 0.16 &              0.44 ± 0.17 &      2 &       0.30 ± 0.11 &          0.08 ± 0.09 &             0.18 ± 0.15 &           0.48 ± 0.18 &             0.44 ± 0.18 \\
numerical_receipe &               phi3 &     starencoder &        0.25 ± 0.08 &           0.04 ± 0.04 &              0.09 ± 0.08 &            0.44 ± 0.17 &              0.44 ± 0.17 &      1 &       0.33 ± 0.13 &          0.11 ± 0.12 &             0.22 ± 0.17 &           0.51 ± 0.19 &             0.45 ± 0.20 \\
numerical_receipe &               phi3 &     starencoder &        0.25 ± 0.08 &           0.04 ± 0.04 &              0.09 ± 0.08 &            0.44 ± 0.17 &              0.44 ± 0.17 &      2 &       0.32 ± 0.12 &          0.10 ± 0.11 &             0.22 ± 0.16 &           0.51 ± 0.19 &             0.45 ± 0.18 \\
numerical_receipe &               phi3 &     starencoder &        0.25 ± 0.08 &           0.04 ± 0.04 &              0.09 ± 0.08 &            0.44 ± 0.17 &              0.44 ± 0.17 &      3 &       0.32 ± 0.12 &          0.09 ± 0.10 &             0.21 ± 0.17 &           0.49 ± 0.19 &             0.46 ± 0.18 \\
numerical_receipe &          starcoder &        codebert &        0.13 ± 0.05 &           0.01 ± 0.01 &              0.01 ± 0.01 &            0.27 ± 0.11 &              0.24 ± 0.18 &      1 &       0.13 ± 0.05 &          0.01 ± 0.01 &             0.01 ± 0.01 &           0.27 ± 0.11 &             0.24 ± 0.18 \\
numerical_receipe &          starcoder &        codebert &        0.13 ± 0.05 &           0.01 ± 0.01 &              0.01 ± 0.01 &            0.27 ± 0.11 &              0.24 ± 0.18 &      2 &       0.13 ± 0.05 &          0.01 ± 0.01 &             0.01 ± 0.01 &           0.27 ± 0.11 &             0.24 ± 0.18 \\
numerical_receipe &          starcoder &        codebert &        0.13 ± 0.05 &           0.01 ± 0.01 &              0.01 ± 0.01 &            0.27 ± 0.11 &              0.24 ± 0.18 &      3 &       0.13 ± 0.05 &          0.01 ± 0.01 &             0.01 ± 0.01 &           0.27 ± 0.11 &             0.25 ± 0.18 \\
numerical_receipe &          starcoder &     nomic_embed &        0.13 ± 0.05 &           0.01 ± 0.01 &              0.01 ± 0.01 &            0.27 ± 0.11 &              0.24 ± 0.18 &      1 &       0.13 ± 0.05 &          0.01 ± 0.01 &             0.01 ± 0.01 &           0.27 ± 0.11 &             0.24 ± 0.18 \\
numerical_receipe &          starcoder &     nomic_embed &        0.13 ± 0.05 &           0.01 ± 0.01 &              0.01 ± 0.01 &            0.27 ± 0.11 &              0.24 ± 0.18 &      2 &       0.13 ± 0.05 &          0.01 ± 0.01 &             0.01 ± 0.01 &           0.27 ± 0.11 &             0.24 ± 0.18 \\
numerical_receipe &          starcoder &     nomic_embed &        0.13 ± 0.05 &           0.01 ± 0.01 &              0.01 ± 0.01 &            0.27 ± 0.11 &              0.24 ± 0.18 &      3 &       0.13 ± 0.05 &          0.01 ± 0.01 &             0.01 ± 0.01 &           0.27 ± 0.11 &             0.25 ± 0.18 \\
numerical_receipe &          starcoder &     starencoder &        0.13 ± 0.05 &           0.01 ± 0.01 &              0.01 ± 0.01 &            0.27 ± 0.11 &              0.25 ± 0.18 &      1 &       0.13 ± 0.05 &          0.01 ± 0.01 &             0.01 ± 0.01 &           0.27 ± 0.11 &             0.24 ± 0.18 \\
numerical_receipe &          starcoder &     starencoder &        0.13 ± 0.05 &           0.01 ± 0.01 &              0.01 ± 0.01 &            0.27 ± 0.11 &              0.25 ± 0.18 &      2 &       0.13 ± 0.05 &          0.01 ± 0.01 &             0.01 ± 0.01 &           0.27 ± 0.11 &             0.24 ± 0.18 \\
numerical_receipe &          starcoder &     starencoder &        0.13 ± 0.05 &           0.01 ± 0.01 &              0.01 ± 0.01 &            0.27 ± 0.11 &              0.25 ± 0.18 &      3 &       0.13 ± 0.05 &          0.01 ± 0.01 &             0.01 ± 0.01 &           0.27 ± 0.12 &             0.25 ± 0.18 \\
\bottomrule
\end{tabular}
